Relative Equilibria and Periodic Orbits in a Binary Asteroid Model

We present a planar four-body model, called the Binary Asteroid Problem, for the motion of two asteroids (having small but positive masses) moving under the gravitational attraction of each other, and under the gravitational attraction of two primaries (with masses much larger than the two asteroids) moving in uniform circular motion about their center of mass. We show the Binary Asteroid Model has (at least) 6 relative equilibria and (at least) 10 one-parameter families of periodic orbits, two of which are of Hill-type. The existence of six relative equilibria and 8 one-parameter families of periodic orbits is obtained by a reduction of the Binary Asteroid Problem in which the primaries have equal mass, the asteroids have equal mass, and the positions of the asteroids are symmetric with respect to the origin. The remaining two one-parameter families of periodic orbits, which are of comet-type, are obtained directly in the Binary Asteroid Problem.

==> references.tex <==
@book{meyerOffin,
  author =  {K. R. Meyer and D. C. Offin},
  title =   {Introduction to Hamiltonian Dynamical Systems and the N-Body Problem},
  editor =    {},
  publisher = {Springer International Publishing},
  year =      {2017},
  volume =    {90},
  number =    {},
  series =    {Applied Mathematical Sciences},
  address =   {},
  edition =   {3rd},
  month =     {},
}

@article{Llibre2021,
  author =  {J. Llibre and D. Pa?ca and C. Valls},
  title =   {The circular restricted 4-body problem with three equal primaries in the collinear central configuration of the 3-body problem},
  journal = {Celestial Mechanics and Dynamical Astronomy},
  year =    {2021},
  volume =  {133},
  number =  {53},
  pages =   {},
  doi =     {https://doi.org/10.1007/s10569-021-10052-6},
}

@article{AlvarezRamirez2015,
  author =  {M. Alvarez-Ram'rez and J.E.F. Skea and T.J. Stuchi},
  title =   {Nonlinear stability analysis in a equilateral restricted four-body problem},
  journal = {Astrophys Space Sci},
  year =    {2015},
  volume =  {358},
  number =  {3},
  pages =   {},
  doi =     {https://doi.org/10.1007/s10509-015-2333-4},
}

@article{Corbera2014,
  author =  {M. Corbera and J. Llibre},
  title =   {Central configurations of the $4$-body problem with masses $m_1=m_2>m_3=m_4>0$ and small},
  journal = {Appl Math Comput},
  year =    {2014},
  volume =  {246},
  number =  {},
  pages =   {121-147},
  doi =     {https://doi.org/10.1016/j.amc.2014.07.109},
}

@article{AlvarezRamirez2013,
  author =  {M. Alvarez-Ram\'irez and J. Llibre},
  title =   {The symmetric central configuration of the $4$-body problem with masses $m_1=m_2\ne m_3=m_4$},
  journal = {Appl Math Comput},
  year =    {2013},
  volume =  {219},
  number =  {},
  pages =   {5996-6001},
  doi =     {https://doi.org/10.1016/j.amc.2012.12.036},
}

@article{Long2002,
  author =  {Y. Long and S. Sun},
  title =   {Four-Body Central Configurations with some Equal Masses},
  journal = {Arch Rational Mech Anal},
  year =    {2002},
  volume =  {162},
  number =  {},
  pages =   {25-44},
  doi =     {https//doi.org/10.1007/s002050100183},
}

@article{Simo,
  author =  {C. Sim\'o},
  title =   {Relative Equilibrium Solutions in the Four Body Problem},
  journal = {Celestial Mechanics},
  year =    {1978},
  volume =  {18},
  number =  {},
  pages =   {165-184},
  doi =     {},
}

@article{Roy,
  author =  {A. E. Roy and B. A. Steves},
  title =   {Some Special restricted four-body problems-{\rm II}: From Caledonia to Copenhagen},
  journal = {Planet Space Sci},
  year =    {1998},
  volume =  {46},
  number =  {11-12},
  pages =   {1475-1486},
  doi =     {},
}

@article{Shoaib,
  author =  {M. Shoaib and I. Faye},
  title =   {Collinear Equilibrium Solutions of Four-Body Problems},
  journal = {J Astrophys Astr},
  volume =  {32},
  year =    {2011},
  number =  {},
  pages =   {411-423},
  doi =     {},
}

@article{Davis,
  author =  {J. Davis},
  title =   {Planetary Society asteroid hunters help find rare type of double asteroid},
  journal = {The Planetary Society},
  year =    {2018},
  number =  {},
  pages =   {},
  note =     {Online article at https://www.planetary.org/articles/shoemaker-winners-2017-ye5},
}

@manual{nasa,
  author =  {C. Cofield and J. Wendel},
  title =   {Observatories Team Up To Reveal Rare Double Asteroid},
  organization = {NASA},
  year =    {2018},
  note =    {Online article at https://www.nasa.gov/feature/jpl/observatories-team-up-to-reveal-rare-double-asteroid},
}

@misc{Johnston,
  author =  {W. R. Johnston},
  title =   {Asteroids with Satellites},
  year =    {2023},
  note =    {Online Database at https://www.johnstonsarchive.net/astro/asteroidmoons.html},
}

@article{Monteiro,
  author =  {F. Monteiro and E. Rond\'on and D. Lazzaro and J. Oey and M Evangelista-Santana and P. Avcoverde and M DeCicco and J. S. Silva-Cabrera and T. Rodrigues and L. B. Santos},
  title =   {Physical characterization of equal-mass binary near-Earth asteroid 2017 YE5: a possible dormant Jupiter-family comet},
  journal = {Monthly Notices of the Royal Astronomical Society},
  year =    {2021},
  volume =  {507},
  number =  {},
  pages =   {5403-5414},
  doi =     {https://doi.org/10.1093/mnras/stab2408},
}

@article{Scheeres,
  author =  {D. J. Scheeres and J. Bellerose},
  title =   {The Restricted Hill Full $4$-Body Problem: application to spacecraft motion about binary asteroids},
  journal = {Dyn Syst},
  year =    {2005},
  volume =  {20},
  number =  {1},
  pages =   {23-44},
  doi =     {https://doi.org/10.1080/1468936042000281321},
}

@article{Wang,
  author =  {H.S. Wang and X. Y. Hou},
  title =   {Forced Hovering orbit above the primary in the binary asteroid system},
  journal = {Celest Mech Dyn Astron},
  year =    {2022},
  volume =  {134},
  number =  {},
  pages =   {},
  doi =     {https://doi.org/10.1007/s10569-022-10098-0},
}

@article{Lu,
  author =  {J. Lu H. Shang and B. Wei},
  title =   {Accelerating binary asteroid system propagation via nested interpolation method},
  journal = {Celest Mech Dyn Astron},
  year =    {2023},
  volume =  {135},
  number =  {},
  pages  =  {},
  doi    =  {https://doi.org/10.1007/s10569-023-10123-w},
}

@article{Espitia,
  author =  {D. Espitia and E. A. Quintero and I. D. Arellano-Ram\'irez},
  title =   {Determination of Orbital Elements and Ephemerides using the Geometric Laplace's Method},
  journal = {J Astron Space Sci},
  year =    {2020},
  volume =  {37},
  number =  {3},
  pages =   {171-185},
  doi =     {https://doi.org/10.5140/JASS.2020.37.3.171},
}

@article{Stoica,
  author =  {J. Llibre and C. Stoica},
  title =   {Comet- and Hill-type periodic orbits in restricted $(N+1)$-body problems},
  journal = {J Differential Equations},
  year =    {2011},
  volume =  {250},
  number =  {},
  pages =   {1747-1766},
  doi =     {doi:10.1016/j.jde.2010.08.005},
}

@unpublished{Bakker,
  author =  {L. F. Bakker and J. Murri and S. Simmons},
  title =   {A model for the Binary Asteroid 2017 YE5},
  year =    {2023},
  Note =    {In preparation},
}

@unpublished{Cochran,
  author =  {L. F. Bakker and S. Cochran},
  title =   {Periodic solutions in the planar $5$-body problem with two free bodies},
  year =    {2021},
  note =    {Undergraduate Research},
}

@misc{Freeman,
  author = {N. J. Freeman},
  title  = {Investigations of a Binary Asteroid Dynamical Model},
  year   = {2023},
  month  = {April},
  note   = {Senior Thesis, Department of Physics and Astronomy, Brigham Young University},
}

@book{Szebehely,
  author    = {V. Szebehely},
  title     = {The Theory of Orbits},
  publisher = {Academic Press},
  address   = {New York},
  year      = {1967},
}



